Lifting 2D Object Locations to 3D by Discounting LiDAR Outliers across Objects and Views

We present a system for automatic converting of 2D mask object predictions and raw LiDAR point clouds into full 3D bounding boxes of objects. Because the LiDAR point clouds are partial, directly fitting bounding boxes to the point clouds is meaningless. Instead, we suggest that obtaining good results requires sharing information between \emph{all} objects in the dataset jointly, over multiple frames. We then make three improvements to the baseline. First, we address ambiguities in predicting the object rotations via direct optimization in this space while still backpropagating rotation prediction through the model. Second, we explicitly model outliers and task the network with learning their typical patterns, thus better discounting them. Third, we enforce temporal consistency when video data is available. With these contributions, our method significantly outperforms previous work despite the fact that those methods use significantly more complex pipelines, 3D models and additional human-annotated external sources of prior information.

==> figures/error_bars.tex <==
\pgfplotstableread{
x       y      y-max  y-min
Easy  79.93 4.16 1.89
Medium 81.14 1.05  1.29
Hard 73.15 0.94 0.92    
}{\mytable}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis} [
                ymin=70,
                rotate=90,
                height=8cm,
                width=3cm,
                symbolic x coords={Easy, Medium, Hard},
                xtick=data,
                yticklabel pos=left,
                xticklabel pos=top,
                xticklabel style={left},
                yticklabel style={top},
                x dir=reverse,
                y dir=reverse
            ]
            \addplot [only marks] 
              plot [error bars/.cd, y dir=both, y explicit]
              table [y error plus=y-max, y error minus=y-min] {\mytable};
            \end{axis} 
    \end{tikzpicture}

    \caption{Error bars showing the variance of our method with 32 yaw bins with varying random seeds with the average, minimum and maximum shown for 14 runs.}
    \label{fig:error_bar}
\end{figure}


==> figures/method/ambiguous.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c c c}
         \includegraphics[height=0.135\textwidth]{figures/method/ambiguous/ex4/rgb.png}
        &\includegraphics[height=0.135\textwidth]{figures/method/ambiguous/ex4/pcd.png} &
         \includegraphics[height=0.135\textwidth]{figures/method/ambiguous/ex6/rgb.png}
        &\includegraphics[height=0.135\textwidth]{figures/method/ambiguous/ex6/pcd.png}
    \end{tabular}
    \caption{In some cases the LiDAR point cloud only captures a single surface of the vehicle. This is problematic as fitting such point clouds is ambiguous, particularly for the rotation component.}\label{fig:ambiguous}
\end{figure}

==> figures/method/outliers.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c c c}

        %  \includegraphics[width=0.2\textwidth]{figures/method/ambiguous/ex2/rgb.png}
        % &\includegraphics[width=0.2\textwidth]{figures/method/ambiguous/ex2/pcd.png} &
         \includegraphics[width=0.2\textwidth]{figures/method/ambiguous/ex3/rgb.png}
        &\includegraphics[width=0.1\textwidth]{figures/method/ambiguous/ex3/pcd.png} % &
        %  \includegraphics[width=0.2\textwidth]{figures/method/ambiguous/ex5/rgb.png}
        % &\includegraphics[width=0.2\textwidth]{figures/method/ambiguous/ex5/pcd.png}
        
    \end{tabular}
    
    \caption{Even with the pixel level Mask-RCNN detections our remaining pointclouds in blue can still have a lot of noise caused occluding objects or imperfect masks which cause problems for a chamfer distance like fit}
    \label{fig:dataset_example}
\vspace{-8mm}
\end{figure}

==> tables/Quantitative.tex <==
\begin{table*}[b]
\newcommand{\zero}{ZERO}
\centering

\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{1.8mm}{
\begin{tabular}{c | c | c c | c | c c c }
 \toprule
 \multirow{2}{*}{Paradigm} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{External Data Supervision} & & \multicolumn{3}{c}{AP\textsubscript{BEV}~/~AP\textsubscript{3D} (IoU = 0.5)} \\
 & & COCO 2D Detection & Pascal3d & Kitti GT 2D Boxes & Easy & Moderate & Hard \\\hline


% \multirow{3}{*}{\textit{\makecell{ Weakly \\ supervised}}}
%   &PCL~\cite{tang2018pcl}      &  & & & 1.878 /- &1.058 /- &0.935 /- \\
%   &OICR~\cite{tang2017oicr}    &  & & & 6.481 /- &2.933 /- &3.270 /- \\
%   &MELM~\cite{wan2018min}      &  & & & 2.796 /- &1.486 /- &1.476 /- \\
%     \hline

\multirow{1}{*}{\textit{\makecell{Supervised}}}
  &Frustum PointNet~\cite{qi2017frustum}      & & & & 98.25/98.10 & 94.92/94.31 & 87.14/86.48 \\
    \hline

%   &VS3D\cite{meng2020ws3d} & Mono   & 2d box,Yaw & 76.93 / 31.35 & 71.84 / 23.92 & 59.39 / 19.34 \\
%   &VS3D\cite{meng2020ws3d} & Stereo & 2d box,Yaw & 79.03 / 40.98 & 72.71 / 34.09 & 59.77 / 27.65 \\

  
   
   
%   &VS3D\cite{meng2020ws3d} & Mono + LiDAR    & Yaw from Image & 81.60 / 41.83 & 72.43 / 39.22 & 64.31 / 32.73 \\
%   &VS3D\cite{meng\2020ws3d} & Stereo + LiDAR  & Yaw from Image & 81.95 / 42.43 & 73.21 / 41.58 & 64.34 / 32.74 \\
%   \hline
  &VS3D\cite{meng2020ws3d} &  & \cellcolor{green} 2D Detection, Yaw & & 74.54 / 40.32 & 66.71 / 37.36 & 57.55 / 31.09 \\ 
  
  
\multirow{3}{*}{\textit{\makecell{Unsupervised}}}
   &Zakharov et al. \cite{sdflabel} & \cellcolor{green}\checkmark & & \cellcolor{green}\checkmark & 77.84/62.25 & 59.75/42.23 & -/- \\
   % Cremers paper here?
   
   &Ours &\cellcolor{green}\checkmark & &  & \textbf{82.37}/\textbf{78.48} & \textbf{82.57}/\textbf{77.63} & \textbf{74.40}/\textbf{69.90} \\
   
\end{tabular}}} 
\label{t:averageprecision}

\caption{Object Detection Average-Precision on the Kitti validation set. Compared to our Method VS3D\cite{meng2020ws3d} uses a network trained on Pascal 3D and NYC 3D Cars\cite{xiang_wacv14, MatzenICCV13} to determine the object Yaw and 2D box, while while Zakharov\cite{sdflabel} only considers MASK R-CNN detections with an IOU > $50\%$ compared to a ground truth box and uses a synthetic dataset to train a network which gives yaw.}

\end{table*}
